Higher-form anomalies and state-operator correspondence beyond conformal invariance

We establish a state-operator correspondence for a class of non-conformal quantum field theories with continuous higher-form symmetries and a mixed anomaly. Such systems can always be realised as a relativistic superfluid. The symmetry structure induces an infinite tower of conserved charges, which we construct explicitly. These charges satisfy an abelian current algebra with a central extension, generalising the familiar Kac-Moody algebras to higher dimensions. States and operators are organised into representations of this algebra, enabling a direct correspondence. We demonstrate the correspondence explicitly in free examples by performing the Euclidean path integral on a $d$-dimensional ball, with local operators inserted in the origin, and matching to energy eigenstates on $S^{d-1}$ obtained by canonical quantisation. Interestingly, in the absence of conformal invariance, the empty path integral prepares a squeezed vacuum rather than the true ground state.

==> preamble.tex <==
%%% Style

% Layout
\RequirePackage[top=12mm,bottom=12mm,left=30mm,right=30mm,head=12mm,includeheadfoot]{geometry}
\bigskipamount 6mm

% For table of contents: remove trailing dots
\RequirePackage{tocloft}
\renewcommand{\cftdot}{}
% Add References to TOC
\RequirePackage[nottoc,notlot,notlof]{tocbibind}

% doi links in references
% \RequirePackage{doi}


\RequirePackage{xcolor}
\RequirePackage{graphicx}


% Font
% Latin Modern
\usepackage{amsfonts,amssymb,amsthm}
\usepackage{upgreek,mathrsfs}
\usepackage{bold-extra}
\usepackage{microtype}


% Patch: add boldface to sections
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother

% Colours
\PassOptionsToPackage{dvipsnames}{xcolor}
\definecolor{maroon}{RGB}{167,74,74}
\definecolor{magreen}{RGB}{59,125,37}
\definecolor{mablue}{RGB}{59,136,195}
\definecolor{mayellow}{RGB}{242,147,24}
\colorlet{mabrown}{maroon!50!magreen}
\colorlet{maorange}{maroon!50!mayellow}
\colorlet{macyan}{magreen!50!mablue}

% Redefine common colours
\colorlet{red}{maroon}
\colorlet{green}{magreen}
\colorlet{blue}{mablue}
\colorlet{yellow}{mayellow}
\colorlet{brown}{mabrown}
\colorlet{orange}{maorange}
\colorlet{cyan}{macyan}

% Extra colours
\definecolor{rred}{RGB}{167,33,74}
\definecolor{bblue}{RGB}{29,136,255}
\definecolor{ppurple}{RGB}{113,84,165}
\definecolor{ppink}{RGB}{255,55,219}

% Custom commands
\newcommand{\blue}[1]{\textcolor{mablue}{#1}}
\newcommand{\red}[1]{\textcolor{maroon}{#1}}
\newcommand{\green}[1]{\textcolor{magreen}{#1}}
\newcommand{\gray}[1]{\textcolor{black!40}{#1}}

% Hyperrefs
\RequirePackage{hyperref}
\hypersetup{colorlinks,
    linkcolor=mablue,
    citecolor=magreen,
    urlcolor=maorange,
    anchorcolor=mablue,
    filecolor=mablue,
    menucolor=mablue}


% No indent paragraphs
\setlength{\parindent}{0em}
\setlength{\parskip}{1em}


%%% Commands and packages

\usepackage{mathtools}
\usepackage{import}
\usepackage{csquotes}
\newcommand{\nn}{\nonumber \\}
\renewcommand{\t}[1]{{\text{#1}}}

\newcommand{\roteqq}{\text{\rotatebox{90}{$=$}}}
\newcommand{\rotequiv}{\text{\rotatebox{90}{$\equiv$}}}
\newcommand{\rotcoloneqq}{\text{\rotatebox{90}{$\coloneqq$}}}
\newcommand{\roteqqcolon}{\text{\rotatebox{90}{$\eqqcolon$}}}
\newcommand{\demeqq}{\overset{!}{=}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}

% Physics
\usepackage{physics}
\newcommand{\parti}{\mathcal{Z}}
\newcommand{\pd}{\partial} % partial derivative
\let\f\relax
\newcommand{\f}[2]{{#1}_{\qty[#2]}} % p-form
\newcommand{\gf}[2]{{#1}^{\qty[#2]}} % p-form group

\newcommand{\inv}[1]{{{#1}^{-1}}} % inverse
\newcommand{\adj}[1]{{#1^{\dagger}}} % adjoint
\newcommand{\trans}[1]{{{#1}^{\top}}} % transpose
\newcommand{\conj}[1]{{#1^*}} % complex conjugate

\usepackage{stackengine}
\newcommand\ccolon{\text{\scalebox{1.2}{\raisebox{0ex}{\stackanchor[.40ex]{.}{.}}}}}
\newcommand{\no}[1]{\; \ccolon {#1} \ccolon \;} %normal ordering

\newcommand{\bm}[1]{\boldsymbol{#1}}

% Maths
\newcommand{\suchthat}{\;\middle|\;}
\renewcommand{\emptyset}{\varnothing}

% reset physics package commands
\renewcommand{\vdot}{\cdot}
\renewcommand{\vnabla}{\nabla}
\renewcommand{\vec}{\boldsymbol}

\newcommand{\w}{\mathbin{\scalebox{0.8}{$\wedge$}}} % wedge
\newcommand{\ex}[1]{\mathrm{e}^{#1}} % e^
\newcommand{\ii}{i} % imaginary i (for consistency in case I want to change style)

\let\C\undefined
\let\U\undefined
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Cx}{\mathbb{C}^{\times}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zx}{\mathbb{Z}^{\times}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\CP}{\mathbb{CP}}
\renewcommand{\S}{S} % sphere (for consistency in case I want to change style)
\newcommand{\B}{B} %ball (for consistency in case I want to change style)
\newcommand{\set}[1]{\qty{#1}}
\newcommand{\eqv}{\Longleftrightarrow}

\newcommand{\U}{\mathrm{U}}
\newcommand{\SU}{\mathrm{SU}}
\renewcommand{\O}{\mathrm{O}}
\newcommand{\SO}{\mathrm{SO}}
\renewcommand{\P}{\mathrm{P}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\Sp}{\mathrm{Sp}}
\newcommand{\alg}[1]{\mathfrak{#1}}
\renewcommand{\sl}{\alg{sl}}
\newcommand{\su}{\alg{su}}
\newcommand{\so}{\alg{so}}
\renewcommand{\sp}{\alg{sp}}
\renewcommand{\u}{\alg{u}}

\renewcommand{\H}{\mathrm{H}} %(co)homology

\newcommand{\blob}{\bullet}
\newcommand{\oblob}{\circ}
\newcommand{\longto}{\longrightarrow}
\newcommand{\xto}[1]{\overset{#1}{\to}}
\renewcommand{\mod}{\ \text{mod}\ }

\makeatletter
\renewcommand{\xmapsto}[2][]{\ext@arrow 0599{\mapstofill@}{#1}{#2}}
\def\mapstofill@{\arrowfill@{\mapstochar\relbar}\relbar\rightarrow}
\makeatother

\let\eval\relax
\newcommand*{\eval}[1]{\left.#1\vphantom{\Big|}\right\rvert}


% \cal, \frak, etc.
% \DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n} % resets mathcal if needed
\def \cA {\mathcal{A}}
\def \cB {\mathcal{B}}
\def \cC {\mathcal{C}}
\def \cD {\mathcal{D}}
\def \cE {\mathcal{E}}
\def \cF {\mathcal{F}}
\def \cG {\mathcal{G}}
\def \cH {\mathcal{H}}
\def \cI {\mathcal{I}}
\def \cJ {\mathcal{J}}
\def \cK {\mathcal{K}}
\def \cL {\mathcal{L}}
\def \cM {\mathcal{M}}
\def \cN {\mathcal{N}}
\def \cO {\mathcal{O}}
\def \cP {\mathcal{P}}
\def \cQ {\mathcal{Q}}
\def \cR {\mathcal{R}}
\def \cS {\mathcal{S}}
\def \cT {\mathcal{T}}
\def \cU {\mathcal{U}}
\def \cV {\mathcal{V}}
\def \cW {\mathcal{W}}
\def \cX {\mathcal{X}}
\def \cY {\mathcal{Y}}
\def \cZ {\mathcal{Z}}

\def \sA {\mathscr{A}}
\def \sB {\mathscr{B}}
\def \sC {\mathscr{C}}
\def \sD {\mathscr{D}}
\def \sE {\mathscr{E}}
\def \sF {\mathscr{F}}
\def \sG {\mathscr{G}}
\def \sH {\mathscr{H}}
\def \sI {\mathscr{I}}
\def \sJ {\mathscr{J}}
\def \sK {\mathscr{K}}
\def \sL {\mathscr{L}}
\def \sM {\mathscr{M}}
\def \sN {\mathscr{N}}
\def \sO {\mathscr{O}}
\def \sP {\mathscr{P}}
\def \sQ {\mathscr{Q}}
\def \sR {\mathscr{R}}
\def \sS {\mathscr{S}}
\def \sT {\mathscr{T}}
\def \sU {\mathscr{U}}
\def \sV {\mathscr{V}}
\def \sW {\mathscr{W}}
\def \sX {\mathscr{X}}
\def \sY {\mathscr{Y}}
\def \sZ {\mathscr{Z}}


% \DeclareMathAlphabet{\mathfrak}{OT1}{pgoth}{m}{n}
% \DeclareMathAlphabet{\mathfrak}{U}{jkpmia}{m}{n} % resets mathfrak if needed
\def \fA {\mathfrak{A}}
\def \fB {\mathfrak{B}}
\def \fC {\mathfrak{C}}
\def \fD {\mathfrak{D}}
\def \fE {\mathfrak{E}}
\def \fF {\mathfrak{F}}
\def \fG {\mathfrak{G}}
\def \fH {\mathfrak{H}}
\def \fI {\mathfrak{I}}
\def \fJ {\mathfrak{J}}
\def \fK {\mathfrak{K}}
\def \fL {\mathfrak{L}}
\def \fM {\mathfrak{M}}
\def \fN {\mathfrak{N}}
\def \fO {\mathfrak{O}}
\def \fP {\mathfrak{P}}
\def \fQ {\mathfrak{Q}}
\def \fR {\mathfrak{R}}
\def \fS {\mathfrak{S}}
\def \fT {\mathfrak{T}}
\def \fU {\mathfrak{U}}
\def \fV {\mathfrak{V}}
\def \fW {\mathfrak{W}}
\def \fX {\mathfrak{X}}
\def \fY {\mathfrak{Y}}
\def \fZ {\mathfrak{Z}}

\def \fa {\mathfrak{a}}
\def \fb {\mathfrak{b}}
\def \fc {\mathfrak{c}}
\def \fd {\mathfrak{d}}
\def \fe {\mathfrak{e}}
\def \ff {\mathfrak{f}}
\def \fg {\mathfrak{g}}
\def \fh {\mathfrak{h}}
\def \fri {\mathfrak{i}} %not \fi (\fi used for if clauses in latex)
\def \fj {\mathfrak{j}}
\def \fk {\mathfrak{k}}
\def \fl {\mathfrak{l}}
\def \fm {\mathfrak{m}}
\def \fn {\mathfrak{n}}
\def \fo {\mathfrak{o}}
\def \fp {\mathfrak{p}}
\def \fq {\mathfrak{q}}
\def \fr {\mathfrak{r}}
\def \fs {\mathfrak{s}}
\def \ft {\mathfrak{t}}
\def \fu {\mathfrak{u}}
\def \fv {\mathfrak{v}}
\def \fw {\mathfrak{w}}
\def \fx {\mathfrak{x}}
\def \fy {\mathfrak{y}}
\def \fz {\mathfrak{z}}

% \DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
% \DeclareSymbolFontAlphabet{\mathbbold}{bbold} % resets mathbb if needed
\def \bbA {\mathbb{A}}
\def \bbB {\mathbb{B}}
\def \bbC {\mathbb{C}}
\def \bbD {\mathbb{D}}
\def \bbE {\mathbb{E}}
\def \bbF {\mathbb{F}}
\def \bbG {\mathbb{G}}
\def \bbH {\mathbb{H}}
\def \bbI {\mathbb{I}}
\def \bbJ {\mathbb{J}}
\def \bbK {\mathbb{K}}
\def \bbL {\mathbb{L}}
\def \bbM {\mathbb{M}}
\def \bbN {\mathbb{N}}
\def \bbO {\mathbb{O}}
\def \bbP {\mathbb{P}}
\def \bbQ {\mathbb{Q}}
\def \bbR {\mathbb{R}}
\def \bbS {\mathbb{S}}
\def \bbT {\mathbb{T}}
\def \bbU {\mathbb{U}}
\def \bbV {\mathbb{V}}
\def \bbW {\mathbb{W}}
\def \bbX {\mathbb{X}}
\def \bbY {\mathbb{Y}}
\def \bbZ {\mathbb{Z}}
\def \bb1 {{\mathbb{1}}}
% \def \bbk {\mathbbold{k}}

\def \sfA {\mathsf{A}}
\def \sfB {\mathsf{B}}
\def \sfC {\mathsf{C}}
\def \sfD {\mathsf{D}}
\def \sfE {\mathsf{E}}
\def \sfF {\mathsf{F}}
\def \sfG {\mathsf{G}}
\def \sfH {\mathsf{H}}
\def \sfI {\mathsf{I}}
\def \sfJ {\mathsf{J}}
\def \sfK {\mathsf{K}}
\def \sfL {\mathsf{L}}
\def \sfM {\mathsf{M}}
\def \sfN {\mathsf{N}}
\def \sfO {\mathsf{O}}
\def \sfP {\mathsf{P}}
\def \sfQ {\mathsf{Q}}
\def \sfR {\mathsf{R}}
\def \sfS {\mathsf{S}}
\def \sfT {\mathsf{T}}
\def \sfU {\mathsf{U}}
\def \sfV {\mathsf{V}}
\def \sfW {\mathsf{W}}
\def \sfX {\mathsf{X}}
\def \sfY {\mathsf{Y}}
\def \sfZ {\mathsf{Z}}

\def \sfa {\mathsf{a}}
\def \sfb {\mathsf{b}}
\def \sfc {\mathsf{c}}
\def \sfd {\mathsf{d}}
\def \sfe {\mathsf{e}}
\def \sff {\mathsf{f}}
\def \sfg {\mathsf{g}}
\def \sfh {\mathsf{h}}
\def \sfi {\mathsf{i}}
\def \sfj {\mathsf{j}}
\def \sfk {\mathsf{k}}
\def \sfl {\mathsf{l}}
\def \sfm {\mathsf{m}}
\def \sfn {\mathsf{n}}
\def \sfo {\mathsf{o}}
\def \sfp {\mathsf{p}}
\def \sfq {\mathsf{q}}
\def \sfr {\mathsf{r}}
\def \sfs {\mathsf{s}}
\def \sft {\mathsf{t}}
\def \sfu {\mathsf{u}}
\def \sfv {\mathsf{v}}
\def \sfw {\mathsf{w}}
\def \sfx {\mathsf{x}}
\def \sfy {\mathsf{y}}
\def \sfz {\mathsf{z}}

% Maths  
\newcommand{\cdd}{\dd^{\dagger}}
% \newcommand{\sd}{\boldsymbol{\dd}}
\newcommand{\lapl}{\Delta}
\newcommand{\tlapl}{\Box}


% Tweaking the {physics} package | needs {xparse}
\def\fdiffd{\mathrm{D}}
\DeclareDocumentCommand\fdifferential{ o g d() }{ % Functional Differential 'D'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
        {\fdiffd\IfNoValueTF{#1}{}{^{#1}}}
        {\mathinner{\fdiffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
    }
    {\mathinner{\fdiffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
}
\DeclareDocumentCommand\DD{}{\fdifferential}

\DeclareDocumentCommand\variation{ o g d() }{ % Functional variation
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(F(g))
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
        {\updelta \IfNoValueTF{#1}{}{^{#1}}}
        {\mathinner{\updelta \IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
    }
    {\mathinner{\updelta \IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
}
\DeclareDocumentCommand\var{}{\variation} % Shorthand for \variation

\def\sdiffd{\mathbf{d}}
\DeclareDocumentCommand\sdifferential{ o g d() }{ % spatial exterior derivative 'd'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
        {\sdiffd\IfNoValueTF{#1}{}{^{#1}}}
        {\mathinner{\sdiffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
    }
    {\mathinner{\sdiffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
}
\DeclareDocumentCommand\sd{}{\sdifferential}

\newcommand{\csd}{\sd^\dagger}

\DeclareDocumentCommand\detp{}{\opbraces{\determinant{}'}}

\DeclareMathOperator{\volume}{vol}
\DeclareDocumentCommand\vol{}{\opbraces{\volume}}

\DeclareMathOperator{\kernel}{ker}
\DeclareDocumentCommand\ker{}{\opbraces{\kernel}}

\DeclareMathOperator{\image}{im}
\DeclareDocumentCommand\im{}{\opbraces{\image}}

\DeclareMathOperator{\cokernel}{coker}
\DeclareDocumentCommand\coker{}{\opbraces{\cokernel}}

\DeclareMathOperator{\spectrum}{spec}
\DeclareDocumentCommand\spec{}{\opbraces{\spectrum}}

\DeclareMathOperator{\spanof}{span}
\DeclareDocumentCommand\spn{}{\opbraces{\spanof}}

\DeclareMathOperator{\character}{ch}
\DeclareDocumentCommand\ch{}{\opbraces{\character}}

\DeclareMathOperator{\harm}{Harm}

\DeclareMathOperator{\homomorphism}{Hom}
\DeclareDocumentCommand\hom{}{\opbraces{\homomorphism}}

\renewcommand{\ordersymbol}{\mathrm{O}}

\renewcommand{\ip}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\pip}[2]{\left\llangle#1,#2\right\rrangle}


\RequirePackage{interval}
\intervalconfig{soft open fences}
\newcommand{\ropen}[2]{\interval[open right]{#1}{#2}}
\newcommand{\lopen}[2]{\interval[open left]{#1}{#2}}
\newcommand{\open}[2]{\interval[open]{#1}{#2}}
\newcommand{\closed}[2]{\interval{#1}{#2}}


% Cleverref
\usepackage[noabbrev]{cleveref}
\newcommand{\crefrangeconjunction}{--}
\crefname{subsection}{subsection}{subsections}
\crefname{equation}{}{}

% Number equations after the sections
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\numberwithin{equation}{section}

% Bibliography
\usepackage[
	style=numeric-comp,
	eprint=true, natbib,
	backend=biber,
	maxbibnames=10,
	giveninits=true,
	sorting=none,
	useprefix=true,
	backref=false,
]{biblatex}

% Format titles in italics
\DeclareFieldFormat*{title}{\emph{#1}}

% Format journal names as upright text
\DeclareFieldFormat*{journaltitle}{#1}

% Remove prefix for the `pages` field in the bibliography
\DeclareFieldFormat{pages}{#1}

% Format author names
\DeclareFieldFormat{labelalpha}{\textsc{#1}}
\renewcommand*{\mkbibnamefamily}[1]{\textsc{#1}}
\renewcommand*{\mkbibnameprefix}[1]{\textsc{#1}}
\renewcommand*{\mkbibnamegiven}[1]{\textsc{#1}}

% Remove the "in:" prefix for articles
\renewbibmacro{in:}{}

% Suppress the display of the `urldate`, `month`, `day`, and `issn` fields
\AtEveryBibitem{\clearfield{urldate}}
\AtEveryBibitem{\clearfield{month}}
\AtEveryBibitem{\clearfield{day}}
\AtEveryBibitem{\clearfield{issn}}
\AtEveryBibitem{\clearfield{version}}
